Techniques for second order convergent weakly-compressible smoothed particle hydrodynamics schemes without boundaries

Despite the many advances in the use of weakly-compressible smoothed particle hydrodynamics (SPH) for the simulation of incompressible fluid flow, it is still challenging to obtain second-order convergence even for simple periodic domains. In this paper we perform a systematic numerical study of convergence and accuracy of kernel-based approximation, discretization operators, and weakly-compressible SPH (WCSPH) schemes. We explore the origins of the errors and issues preventing second-order convergence despite having a periodic domain. Based on the study, we propose several new variations of the basic WCSPH scheme that are all second-order accurate. Additionally, we investigate the linear and angular momentum conservation property of the WCSPH schemes. Our results show that one may construct accurate WCSPH schemes that demonstrate second-order convergence through a judicious choice of kernel, smoothing length, and discretization operators in the discretization of the governing equations.

==> figures/compare_c0/compare_c0_100.0_l1_err.tex <==
\begin{tabular}{cllllll}
\toprule
 Resolution & L-IPST-C $c_o=20$ & L-IPST-C $c_o=40$ & L-IPST-C $c_o=80$ & L-IPST-F $c_o=20$ & L-IPST-F $c_o=40$ & L-IPST-F $c_o=80$ \\
\midrule
         50 &          4.68e-03 &          4.59e-03 &          4.52e-03 &          1.34e-03 &          1.27e-03 &          1.24e-03 \\
        100 &    1.25e-03(1.90) &    1.17e-03(1.97) &    1.15e-03(1.97) &    4.30e-04(1.64) &    3.29e-04(1.95) &    3.06e-04(2.01) \\
        200 &    4.13e-04(1.60) &    3.15e-04(1.89) &    2.95e-04(1.96) &    2.25e-04(0.93) &    1.01e-04(1.70) &    7.28e-05(2.07) \\
        250 &    3.18e-04(1.17) &    2.12e-04(1.76) &    1.92e-04(1.92) &    2.05e-04(0.43) &    7.74e-05(1.19) &    4.56e-05(2.10) \\
        400 &    2.23e-04(0.76) &    1.03e-04(1.53) &    7.92e-05(1.89) &    1.84e-04(0.23) &    5.32e-05(0.80) &    1.90e-05(1.86) \\
        500 &    2.03e-04(0.41) &    7.94e-05(1.18) &    5.32e-05(1.78) &    1.80e-04(0.11) &    4.81e-05(0.45) &    1.36e-05(1.50) \\
\bottomrule
\end{tabular}


==> figures/compare_c0/compare_c0_100.0_p_l1_err.tex <==
\begin{tabular}{cllllll}
\toprule
 Resolution & L-IPST-C $c_o=20$ & L-IPST-C $c_o=40$ & L-IPST-C $c_o=80$ & L-IPST-F $c_o=20$ & L-IPST-F $c_o=40$ & L-IPST-F $c_o=80$ \\
\midrule
         50 &          3.11e-02 &          7.57e-02 &          2.04e-01 &          2.10e-02 &          4.97e-02 &          1.50e-01 \\
        100 &    9.88e-03(1.65) &    2.32e-02(1.71) &    6.44e-02(1.66) &    7.96e-03(1.40) &    1.61e-02(1.63) &    4.86e-02(1.62) \\
        200 &    4.49e-03(1.14) &    6.94e-03(1.74) &    1.77e-02(1.86) &    4.61e-03(0.79) &    6.01e-03(1.42) &    1.45e-02(1.74) \\
        250 &    4.01e-03(0.50) &    4.72e-03(1.72) &    1.15e-02(1.92) &    4.23e-03(0.39) &    4.42e-03(1.38) &    1.00e-02(1.67) \\
        400 &    3.69e-03(0.18) &    2.47e-03(1.38) &    4.55e-03(1.98) &    3.84e-03(0.20) &    2.87e-03(0.92) &    4.67e-03(1.62) \\
        500 &    3.66e-03(0.04) &    2.09e-03(0.76) &    2.98e-03(1.90) &    3.77e-03(0.09) &    2.54e-03(0.55) &    3.52e-03(1.26) \\
\bottomrule
\end{tabular}


==> figures/compare_variation/compare_variation_100.0_l1_err.tex <==
\begin{tabular}{clllllll}
\toprule
 Resolution &       L-IPST-C &      PE-IPST-C &            TV-C &        L-PST-C &            E-C &         L-RR-C &         EWCSPH \\
\midrule
         50 &       4.52e-03 &       4.52e-03 &        1.65e-02 &       4.88e-03 &       4.36e-03 &       3.04e-03 &       1.10e-03 \\
        100 & 1.15e-03(1.97) & 1.15e-03(1.98) &  4.75e-03(1.80) & 1.40e-03(1.80) & 1.10e-03(1.99) & 7.68e-04(1.99) & 2.83e-04(1.96) \\
        200 & 2.95e-04(1.96) & 2.93e-04(1.97) &  1.28e-03(1.89) & 3.87e-04(1.86) & 2.80e-04(1.98) & 1.96e-04(1.97) & 8.07e-05(1.81) \\
        250 & 1.92e-04(1.92) & 1.89e-04(1.95) & 1.30e-03(-0.06) & 2.52e-04(1.92) & 1.81e-04(1.95) & 1.28e-04(1.92) & 5.76e-05(1.51) \\
        400 & 7.92e-05(1.89) & 7.64e-05(1.93) &  1.64e-04(4.41) & 1.05e-04(1.87) & 7.49e-05(1.88) & 5.41e-05(1.83) & 3.55e-05(1.03) \\
        500 & 5.32e-05(1.78) & 5.05e-05(1.86) &  1.06e-04(1.95) & 7.31e-05(1.61) & 5.11e-05(1.72) & 3.74e-05(1.66) & 3.25e-05(0.40) \\
\bottomrule
\end{tabular}


==> figures/compare_variation/compare_variation_100.0_p_l1_err.tex <==
\begin{tabular}{clllllll}
\toprule
 Resolution &       L-IPST-C &      PE-IPST-C &            TV-C &        L-PST-C &            E-C &         L-RR-C &          EWCSPH \\
\midrule
         50 &       2.04e-01 &       2.02e-01 &        2.20e+00 &       3.97e-01 &       8.31e-03 &       4.53e-03 &        7.30e-03 \\
        100 & 6.44e-02(1.66) & 6.54e-02(1.62) &  5.54e-01(1.99) & 1.30e-01(1.61) & 2.65e-03(1.65) & 1.42e-03(1.68) & 7.42e-03(-0.02) \\
        200 & 1.77e-02(1.86) & 1.79e-02(1.87) &  1.53e-01(1.86) & 3.94e-02(1.72) & 1.59e-03(0.73) & 9.59e-04(0.56) & 8.86e-03(-0.26) \\
        250 & 1.15e-02(1.92) & 1.15e-02(1.95) & 1.90e-01(-0.99) & 2.60e-02(1.86) & 1.54e-03(0.15) & 9.34e-04(0.12) & 9.31e-03(-0.22) \\
        400 & 4.55e-03(1.98) & 4.58e-03(1.97) &  2.06e-02(4.73) & 1.17e-02(1.69) & 1.50e-03(0.05) & 9.15e-04(0.05) & 1.05e-02(-0.27) \\
        500 & 2.98e-03(1.90) & 3.01e-03(1.89) &  1.51e-02(1.41) & 8.93e-03(1.22) & 1.50e-03(0.01) & 9.11e-04(0.02) & 1.13e-02(-0.31) \\
\bottomrule
\end{tabular}


==> figures/compare_variation/compare_variation_1000.0_time.tex <==
\begin{tabular}{cllll}
\toprule
    Name & $\frac{F_T}{F_{max}}$ & $T_r$ & $L_1(|\ten{u}|)(O)$ &    $L_1(p)(O)$ \\
\midrule
L-IPST-C &              1.27e-05 &   1.0 &      4.52e-09(2.35) & 7.92e-06(0.13) \\
\bottomrule
\end{tabular}


==> figures/div_sph/QuinticSpline_derv1_pert0.tex <==
\begin{tabular}{clll}
\toprule
         Name & $\frac{F_T}{F_{max}}$ & $T_{r}$ &       $L_1(O)$ \\
\midrule
\nam{div\_bc} &                  0.00 &    1.00 & 8.78e-04(2.00) \\
    \nam{div} &                 -0.00 &    1.49 & 5.39e-03(0.39) \\
\bottomrule
\end{tabular}


==> figures/div_sph/QuinticSpline_derv1_pert1.tex <==
\begin{tabular}{clll}
\toprule
         Name & $\frac{F_T}{F_{max}}$ & $T_{r}$ &       $L_1(O)$ \\
\midrule
\nam{div\_bc} &                 -1.68 &    3.74 & 8.88e-04(1.98) \\
    \nam{div} &                 -1.61 &    1.00 & 6.62e-03(0.01) \\
\bottomrule
\end{tabular}


==> figures/div_sph_zero_div/QuinticSpline_derv1_pert0.tex <==
\begin{tabular}{cllll}
\toprule
         Name & $\frac{F_T}{F_{max}}$ & $T_{r}$ & $L_1$ error & Order \\
\midrule
\nam{div\_bc} &              4.13e-01 &    2.26 &    2.18e-14 & -1.15 \\
    \nam{div} &             -3.39e-01 &    1.00 &    2.32e-14 & -0.95 \\
\bottomrule
\end{tabular}


==> figures/div_sph_zero_div/QuinticSpline_derv1_pert1.tex <==
\begin{tabular}{cllll}
\toprule
         Name & $\frac{F_T}{F_{max}}$ & $T_{r}$ & $L_1$ error & Order \\
\midrule
\nam{div\_bc} &              7.30e-02 &    1.94 &    4.24e-05 &  1.03 \\
    \nam{div} &             -7.43e-01 &    1.00 &    2.91e-03 &  0.05 \\
\bottomrule
\end{tabular}


==> figures/grad_sph/QuinticSpline_derv1_pert0.tex <==
\begin{tabular}{clll}
\toprule
          Name & $\frac{F_T}{F_{max}}$ & $T_{r}$ &       $L_1(O)$ \\
\midrule
\nam{asym\_bc} &                  0.00 &    2.16 & 4.39e-04(2.00) \\
    \nam{asym} &                  0.00 &    1.24 & 2.69e-03(0.39) \\
\nam{sym1\_bc} &                  0.00 &    2.31 & 4.39e-04(2.00) \\
\nam{sym1\_lc} &                  0.00 &    2.73 & 4.39e-04(2.00) \\
    \nam{sym1} &                 -0.00 &    1.15 & 2.69e-03(0.39) \\
\nam{sym2\_bc} &                  0.00 &    2.14 & 4.39e-04(2.00) \\
\nam{sym2\_lc} &                  0.00 &    2.70 & 2.69e-03(0.39) \\
    \nam{sym2} &                  0.00 &    1.00 & 2.69e-03(0.39) \\
 \nam{sym\_sl} &                  0.00 &    2.94 & 4.39e-04(2.00) \\
\bottomrule
\end{tabular}


==> figures/laplace_sph/QuinticSpline_derv1_pert0.tex <==
\begin{tabular}{cllll}
\toprule
             Name & $\frac{F_T}{F_{max}}$ & $T_{r}$ & $L_1$ error & Order \\
\midrule
 \nam{Cleary\_bc} &             -6.37e-12 &    2.04 &    5.49e-05 &  2.00 \\
 \nam{Cleary\_lc} &              8.98e-13 &    2.58 &    5.49e-05 &  2.00 \\
     \nam{Cleary} &              1.16e-11 &    1.00 &    6.18e-04 &  0.98 \\
  \nam{Fatehi\_c} &              6.19e-12 &    4.19 &    5.49e-05 &  2.00 \\
     \nam{Fatehi} &             -1.88e-12 &    2.81 &    6.18e-04 &  0.98 \\
  \nam{Korzilius} &              7.13e-12 &    5.04 &    1.10e-04 &  2.00 \\
\nam{coupled\_bc} &              7.30e-12 &    3.25 &    2.20e-04 &  2.00 \\
    \nam{coupled} &              1.15e-11 &    2.51 &    7.83e-04 &  1.47 \\
    \nam{tvf\_bc} &             -2.15e-11 &    1.99 &    7.71e-03 &  0.21 \\
    \nam{tvf\_lc} &             -1.45e-11 &    2.68 &    7.71e-03 &  0.21 \\
        \nam{tvf} &             -1.06e-11 &    1.00 &    8.27e-03 &  0.20 \\
\bottomrule
\end{tabular}


==> figures/scheme_compare/scheme_compare_100.0_l1_err.tex <==
\begin{tabular}{clllll}
\toprule
 Resolution &             TVF & $\delta^{+}SPH$ &            EDAC &       L-IPST-C &          EWCSPH \\
\midrule
         50 &        1.25e-04 &        5.70e-05 &        1.33e-06 &       3.19e-06 &        8.16e-07 \\
        100 & 2.08e-04(-0.73) & 5.71e-05(-0.00) &  7.86e-07(0.76) & 5.68e-07(2.49) &  3.98e-07(1.04) \\
        200 & 4.02e-04(-0.95) & 5.71e-05(-0.00) & 2.71e-06(-1.78) & 1.83e-07(1.63) &  3.22e-07(0.31) \\
        250 & 4.73e-04(-0.73) &  5.71e-05(0.00) & 3.82e-06(-1.54) & 1.49e-07(0.91) &  3.16e-07(0.09) \\
        400 & 7.58e-04(-1.00) &  5.70e-05(0.00) & 1.18e-05(-2.40) & 1.22e-07(0.43) &  3.12e-07(0.03) \\
        500 & 9.45e-04(-0.99) &  5.69e-05(0.01) & 1.68e-05(-1.59) & 1.18e-07(0.16) & 3.13e-07(-0.02) \\
\bottomrule
\end{tabular}


==> figures/scheme_compare/scheme_compare_100.0_p_l1_err.tex <==
\begin{tabular}{clllll}
\toprule
 Resolution &             TVF & $\delta^{+}SPH$ &            EDAC &        L-IPST-C &          EWCSPH \\
\midrule
         50 &        2.46e-01 &        2.03e-01 &        6.07e-05 &        6.47e-05 &        2.11e-05 \\
        100 & 2.66e-01(-0.11) &  2.03e-01(0.00) & 6.25e-05(-0.04) &  6.40e-05(0.01) &  2.10e-05(0.00) \\
        200 & 2.92e-01(-0.14) &  2.03e-01(0.00) & 6.63e-05(-0.08) & 6.40e-05(-0.00) &  2.10e-05(0.00) \\
        250 &  2.87e-01(0.08) & 2.03e-01(-0.00) & 6.70e-05(-0.05) & 6.40e-05(-0.00) &  2.10e-05(0.00) \\
        400 &  2.87e-01(0.00) &  2.03e-01(0.00) & 6.93e-05(-0.07) & 6.41e-05(-0.00) & 2.10e-05(-0.00) \\
        500 & 2.88e-01(-0.01) &  2.03e-01(0.00) & 7.00e-05(-0.05) & 6.41e-05(-0.00) & 2.10e-05(-0.00) \\
\bottomrule
\end{tabular}

